General-relativistic precession in a black-hole binary

The general-relativistic phenomenon of spin-induced orbital precession has not yet been observed in strong-field gravity. Gravitational-wave observations of binary black holes (BBHs) are prime candidates, since we expect the astrophysical binary population to contain precessing binaries. Imprints of precession have been investigated in several signals, but no definitive identification of orbital precession has been reported in any one of the 84 BBH observations to date by the Advanced LIGO and Virgo detectors. Here we report the measurement of strong-field precession in the LIGO-Virgo-Kagra (LVK) gravitational-wave signal GW200129. The binary's orbit precesses at a rate ten orders of magnitude faster than previous weak-field measurements from binary pulsars. We also find that the primary black hole is likely highly spinning. According to current binary population estimates a GW200129-like signal is extremely unlikely, and therefore presents a direct challenge to many current binary formation models.

==> latex_macros.tex <==
\newcommand{\PrimaryMass}{\ensuremath{39_{-7}^{+6}}}
\newcommand{\PrimaryMassMedian}{39.0}
\newcommand{\PrimaryMassUpper}{45.04}
\newcommand{\PrimaryMassLower}{32.16}
\newcommand{\SecondaryMass}{\ensuremath{22_{-4}^{+8}}}
\newcommand{\SecondaryMassMedian}{22.3}
\newcommand{\SecondaryMassUpper}{29.93}
\newcommand{\SecondaryMassLower}{18.5}
\newcommand{\ChirpMass}{\ensuremath{26_{-1}^{+2}}}
\newcommand{\ChirpMassMedian}{26.0}
\newcommand{\ChirpMassUpper}{27.68}
\newcommand{\ChirpMassLower}{24.33}
\newcommand{\TotalMass}{\ensuremath{62_{-3}^{+3}}}
\newcommand{\TotalMassMedian}{62.1}
\newcommand{\TotalMassUpper}{65.34}
\newcommand{\TotalMassLower}{59.48}
\newcommand{\MassRatio}{\ensuremath{0.6_{-0.2}^{+0.4}}}
\newcommand{\MassRatioMedian}{0.6}
\newcommand{\MassRatioUpper}{0.93}
\newcommand{\MassRatioLower}{0.41}
\newcommand{\PrimarySpin}{\ensuremath{0.9_{-0.5}^{+0.1}}}
\newcommand{\PrimarySpinMedian}{0.9}
\newcommand{\PrimarySpinUpper}{0.99}
\newcommand{\PrimarySpinLower}{0.42}
\newcommand{\SecondarySpin}{\ensuremath{0.5_{-0.4}^{+0.5}}}
\newcommand{\SecondarySpinMedian}{0.5}
\newcommand{\SecondarySpinUpper}{0.95}
\newcommand{\SecondarySpinLower}{0.05}
\newcommand{\PrimaryTilt}{\ensuremath{1.4_{-0.5}^{+0.4}}}
\newcommand{\PrimaryTiltMedian}{1.4}
\newcommand{\PrimaryTiltUpper}{1.78}
\newcommand{\PrimaryTiltLower}{0.95}
\newcommand{\SecondaryTilt}{\ensuremath{2_{-1}^{+1}}}
\newcommand{\SecondaryTiltMedian}{2.0}
\newcommand{\SecondaryTiltUpper}{2.76}
\newcommand{\SecondaryTiltLower}{0.55}
\newcommand{\ChiP}{\ensuremath{0.9_{-0.4}^{+0.1}}}
\newcommand{\ChiPMedian}{0.9}
\newcommand{\ChiPUpper}{0.98}
\newcommand{\ChiPLower}{0.48}
\newcommand{\RhoP}{\ensuremath{4_{-2}^{+3}}}
\newcommand{\RhoPMedian}{4.0}
\newcommand{\RhoPUpper}{6.04}
\newcommand{\RhoPLower}{1.06}
\newcommand{\ChiEff}{\ensuremath{0.06_{-0.12}^{+0.13}}}
\newcommand{\ChiEffMedian}{0.06}
\newcommand{\ChiEffUpper}{0.18}
\newcommand{\ChiEffLower}{-0.07}
\newcommand{\Distance}{\ensuremath{1000_{-200}^{+200}}}
\newcommand{\DistanceMedian}{1000.0}
\newcommand{\DistanceUpper}{1213.34}
\newcommand{\DistanceLower}{794.52}
\newcommand{\Redshift}{\ensuremath{0.21_{-0.04}^{+0.03}}}
\newcommand{\RedshiftMedian}{0.21}
\newcommand{\RedshiftUpper}{0.24}
\newcommand{\RedshiftLower}{0.16}
\newcommand{\ThetaJN}{\ensuremath{0.5_{-0.3}^{+0.3}}}
\newcommand{\ThetaJNMedian}{0.5}
\newcommand{\ThetaJNUpper}{0.8}
\newcommand{\ThetaJNLower}{0.22}
\newcommand{\NetworkSNR}{\ensuremath{26.9_{-0.2}^{+0.2}}}
\newcommand{\NetworkSNRMedian}{26.9}
\newcommand{\NetworkSNRUpper}{27.05}
\newcommand{\NetworkSNRLower}{26.62}
\newcommand{\NumberOfSamples}{\ensuremath{1.93 \times 10^5}}
\newcommand{\LSNR}{20.95}
\newcommand{\HSNR}{14.79}
\newcommand{\VSNR}{6.65}
\newcommand{\NetworkSNRunc}{\ensuremath{26.41^{+0.2}_{-0.24}}}
\newcommand{\NetworkSNRgwtc}{26.5}
\newcommand{\LSNRgwtc}{21.2}
\newcommand{\HSNRgwtc}{14.6}
\newcommand{\VSNRgwtc}{6.3}

